PersLay: A Neural Network Layer for Persistence Diagrams and New Graph Topological Signatures

Persistence diagrams, the most common descriptors of Topological Data Analysis, encode topological properties of data and have already proved pivotal in many different applications of data science. However, since the (metric) space of persistence diagrams is not Hilbert, they end up being difficult inputs for most Machine Learning techniques. To address this concern, several vectorization methods have been put forward that embed persistence diagrams into either finite-dimensional Euclidean space or (implicit) infinite dimensional Hilbert space with kernels. In this work, we focus on persistence diagrams built on top of graphs. Relying on extended persistence theory and the so-called heat kernel signature, we show how graphs can be encoded by (extended) persistence diagrams in a provably stable way. We then propose a general and versatile framework for learning vectorizations of persistence diagrams, which encompasses most of the vectorization techniques used in the literature. We finally showcase the experimental strength of our setup by achieving competitive scores on classification tasks on real-life graph datasets.

==> tables/tableau_res_save_May.tex <==
%\theo{If you change something in the column Spectral + HKS + TDA , first congrats, you beat our best score, second, you must describe the method used in the \texttt{tables/expe\_settings.tex} table.}

\begin{table}
\begin{center}

\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|cccc||cc|}
\hline
	Dataset   & ScaleVariant\footnotemark[1] & RetGK1 \bf{*} \footnotemark[2] & RetGK11 \bf{*} \footnotemark[2] & FGSD \footnotemark[3] & Spectral + HKS \footnotemark[4] & PersLay \\
\hline
% Social network datasets
	$\texttt{REDDIT5K}$        & ---  & 56.1($\pm$0.5) & 55.3($\pm$0.3) & 47.8 & 49.7($\pm$0.3) & \textbf{56.6}($\pm$0.3) \\
	$\texttt{REDDIT12K}$       & ---  & \textbf{48.7}($\pm$0.2) & 47.1($\pm$0.3) & ---  & 39.7($\pm$0.1) & 47.7($\pm$0.2) \\
	$\texttt{COLLAB}$          & ---  & \textbf{81.0($\pm$0.3)} & 80.6($\pm$0.3) & 80.0 & 67.8($\pm$0.2) & 76.4($\pm$0.4) \\
	$\texttt{IMDB-B}$          & 72.9 & 71.9($\pm$1.0) & 72.3($\pm$0.6) & \textbf{73.6} & 67.6($\pm$0.6) & 70.9($\pm$0.7) \\
	$\texttt{IMDB-M}$          & 50.3 & 47.7($\pm$0.3) & 48.7($\pm$0.6) & \textbf{52.4} & 44.5($\pm$0.4) & 48.7($\pm$0.6) \\
% Bio informatic datasets
	$\texttt{BZR}$ \bf{*}      & 86.6 & ---  & --- & ---  & 80.8($\pm$0.8) & \textcolor{blue}{\textbf{87.2($\pm$0.7)}} \\
	$\texttt{COX2}$ \bf{*}     & 78.4 & 80.1($\pm$0.9) & 81.4($\pm$0.6) & ---  & 78.2($\pm$1.3) & \textcolor{blue}{\textbf{81.6($\pm$1.0)}} \\
	$\texttt{DHFR}$ \bf{*}     & 78.4 & 81.5($\pm$0.9) & \textbf{82.5($\pm$0.8)} & ---  & 69.5($\pm$1.0) & \textcolor{blue}{81.8($\pm$0.8)} \\
	$\texttt{MUTAG}$ \bf{*}    & 88.3 & 90.3($\pm$1.1) & 90.1($\pm$1.0)          & \textcolor{blue}{\textbf{92.1}} & 85.8($\pm$1.3) & 89.8($\pm$0.9) \\
	$\texttt{PROTEINS}$ \bf{*} & 72.6 & \textbf{75.8($\pm$0.6)} & 75.2($\pm$0.3) & 73.4 & 73.5($\pm$0.3) & \textcolor{blue}{74.8($\pm$0.3)} \\
% New datasets recently added, to insert in correct line
	$\texttt{NCI1}$ \bf{*}     & 71.6 & \textbf{84.5($\pm$0.2)} & 83.5($\pm$0.2)          & \textcolor{blue}{79.8} & 65.3($\pm0.2$) & 72.8($\pm$0.3) \\
	$\texttt{NCI109}$ \bf{*}   & 70.5 & ---  &   ---                   & \textcolor{blue}{\textbf{78.8}} & 64.9($\pm$0.2) & 71.7($\pm$0.3) \\
	$\texttt{FRANKENSTEIN}$    & 69.4 & ---  &   ---                   & ---  & 62.9($\pm$0.1) & \textbf{70.7($\pm$0.4)} \\
\hline
\end{tabular}}
\end{center}
\caption[Caption for result]{Mean accuracies and standard deviations over ten 10-folds, for \citep{zhang2018retgk}\footnotemark[2] and our own evaluations (right hand side). In \citep{tran2018scale}\footnotemark[1] the average accuracy over 100 random splits at different proportions of training data is reported, and in \citep{verma2017hunt}\footnotemark[3] the mean accuracy over a single 10-fold is reported. The \textbf{*} indicates those datasets that contain attributes (labels) on graph nodes and symmetrically the methods that leverage such attributes for classification purposes. Blue color represents the best method that does not use node attributes (when there are), and bold fonts mark the overall best score on a given problem.}
\label{tab:tableau_res}
\end{table}


==> tables/tableau_res_save_Sept.tex <==
%\theo{If you change something in the column Spectral + HKS + TDA , first congrats, you beat our best score, second, you must describe the method used in the \texttt{tables/expe\_settings.tex} table.}

\begin{table*}
\begin{center}

\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|ccccc||cc|}
\hline
	Dataset   & ScaleVariant\footnotemark[1] & RetGK1 \bf{*} \footnotemark[2] & RetGK11 \bf{*} \footnotemark[2] & FGSD \footnotemark[3] & GCNN \footnotemark[4] & Spectral + HKS \footnotemark[5] & PersLay \\
\hline
% Social network datasets
	$\texttt{REDDIT5K}$        & ---  & 56.1($\pm$0.5) & 55.3($\pm$0.3) & 47.8 & 52.9 & 49.7($\pm$0.3) & \textbf{56.6}($\pm$0.3) \\
	$\texttt{REDDIT12K}$       & ---  & \textbf{48.7}($\pm$0.2) & 47.1($\pm$0.3) & ---  & 46.6 & 39.7($\pm$0.1) & 47.7($\pm$0.2) \\
	$\texttt{COLLAB}$          & ---  & \textbf{81.0($\pm$0.3)} & 80.6($\pm$0.3) & 80.0 & 79.6 & 67.8($\pm$0.2) & 76.4($\pm$0.4) \\
	$\texttt{IMDB-B}$          & 72.9 & 71.9($\pm$1.0) & 72.3($\pm$0.6) & \textbf{73.6} & 73.1 & 67.6($\pm$0.6) & 70.9($\pm$0.7) \\
	$\texttt{IMDB-M}$          & 50.3 & 47.7($\pm$0.3) & 48.7($\pm$0.6) & \textbf{52.4} & 50.3 & 44.5($\pm$0.4) & 48.7($\pm$0.6) \\
% Bio informatic datasets
	$\texttt{BZR}$ \bf{*}      & 86.6 & ---  & --- & ---  & --- & 80.8($\pm$0.8) & \textcolor{blue}{\textbf{87.2($\pm$0.7)}} \\
	$\texttt{COX2}$ \bf{*}     & 78.4 & 80.1($\pm$0.9) & 81.4($\pm$0.6) & --- & --- & 78.2($\pm$1.3) & \textcolor{blue}{\textbf{81.6($\pm$1.0)}} \\
	$\texttt{DHFR}$ \bf{*}     & 78.4 & 81.5($\pm$0.9) & \textbf{82.5($\pm$0.8)} & ---  & --- & 69.5($\pm$1.0) & \textcolor{blue}{81.8($\pm$0.8)} \\
	$\texttt{MUTAG}$ \bf{*}    & 88.3 & 90.3($\pm$1.1) & 90.1($\pm$1.0)          & \textcolor{blue}{\textbf{92.1}} & 86.7 & 85.8($\pm$1.3) & 89.8($\pm$0.9) \\
	$\texttt{PROTEINS}$ \bf{*} & 72.6 & 75.8($\pm$0.6) & 75.2($\pm$0.3) & 73.4 & \textbf{76.3} & 73.5($\pm$0.3) & \textcolor{blue}{74.8($\pm$0.3)} \\
	$\texttt{NCI1}$ \bf{*}     & 71.6 & \textbf{84.5($\pm$0.2)} & 83.5($\pm$0.2) & \textcolor{blue}{79.8} & 78.4 & 65.3($\pm0.2$) & 72.8($\pm$0.3) \\
	$\texttt{NCI109}$ \bf{*}   & 70.5 & ---  &   ---                   & \textcolor{blue}{\textbf{78.8}} & --- & 64.9($\pm$0.2) & 71.7($\pm$0.3) \\
	$\texttt{FRANKENSTEIN}$    & 69.4 & ---  &   ---                   & --- & --- & 62.9($\pm$0.1) & \textbf{70.7($\pm$0.4)} \\
\hline
\end{tabular}}
\end{center}
\caption[Caption for result]{Mean accuracies and standard deviations over ten 10-folds, for \citep{zhang2018retgk}\footnotemark[2] and our own evaluations (right hand side). In \citep{tran2018scale}\footnotemark[1] the average accuracy over 100 random splits at different proportions of training data is reported, and in \citep{verma2017hunt}\footnotemark[3] and \citep{xinyi2018capsule}\footnotemark[4] the mean accuracy over a single 10-fold is reported. The \textbf{*} indicates those datasets that contain attributes (labels) on graph nodes and symmetrically the methods that leverage such attributes for classification purposes. Blue color represents the best method that does not use node attributes (when there are), and bold fonts mark the overall best score on a given problem.}
\label{tab:tableau_res}
\end{table*}

